Shape from Semantics: 3D Shape Generation from Multi-View Semantics

Existing 3D reconstruction methods utilize guidances such as 2D images, 3D point clouds, shape contours and single semantics to recover the 3D surface, which limits the creative exploration of 3D modeling. In this paper, we propose a novel 3D modeling task called ``Shape from Semantics'', which aims to create 3D models whose geometry and appearance are consistent with the given text semantics when viewed from different views. The reconstructed 3D models incorporate more than one semantic elements and are easy for observers to distinguish. We adopt generative models as priors and disentangle the connection between geometry and appearance to solve this challenging problem. Specifically, we propose Local Geometry-Aware Distillation (LGAD), a strategy that employs multi-view normal-depth diffusion priors to complete partial geometries, ensuring realistic shape generation. We also integrate view-adaptive guidance scales to enable smooth semantic transitions across views. For appearance modeling, we adopt physically based rendering to generate high-quality material properties, which are subsequently baked into fabricable meshes. Extensive experimental results demonstrate that our method can generate meshes with well-structured, intricately detailed geometries, coherent textures, and smooth transitions, resulting in visually appealing 3D shape designs. Project page: https://shapefromsemantics.github.io

==> figures/fig_comparison.tex <==
\begin{figure}[ht]
    % \raggedleft
    \centering
    \includegraphics[width=0.45\textwidth]{figures/ShadowArt.pdf}
    % \setlength{\abovecaptionskip}{2pt} 
    \caption{\textbf{Comparison with different multi-view inverse design problems.} We compare with shadow art \cite{MP09}, wire art \cite{Fabricable3DWireArt}. Considering that the input for shadow art is a given image, the inputs for shadow art and wire art during comparison are respectively the masks and RGB images derived from the observation views restored in \ref{3_2}. The input views are [0,0], [0,90], [-90,0]. The results illustrate that our models effectively integrate multiple semantic elements, presenting the information in a manner that is more readily perceivable to observers. }
    \label{fig:ShadowArt}
\end{figure}

\begin{figure}[ht]
    % \raggedleft
    \centering
    \includegraphics[width=0.45\textwidth]{figures/experiments/WireArt.pdf}
    % \setlength{\abovecaptionskip}{2pt} 
    \caption{\textbf{Comparison with wire art \cite{Fabricable3DWireArt}.} We input semantics for comparison. The first-line result highlights the angular limitations of Wire Art, which arise from its dependence on shadows to convey information. All results demonstrate that our model not only captures perceptual 3D characteristics but also offers high levels of creativity, visual appeal, and engagement.}
    \label{fig:wireArt}
\end{figure}

==> figures/fig_fab.tex <==
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figures/fab_results.pdf}
%   \caption{\textbf{Gallery of Shape from Semantics}. We show the input to our method, the generated colored mesh, the rendering and normal results of each semantics. The normal maps show that our generated shape has meaningful geometry aligned with the rendering.}
%   \label{fig:fab}
% \end{figure*}
\begin{figure}[t]
    % \raggedleft
    \centering
    \includegraphics[width=0.41\textwidth]{figures/experiments/fab_results.pdf}
    \setlength{\abovecaptionskip}{2pt} 
    \caption{\textbf{Fabrication results.} Results show that the manufactured outcomes are nearly identical to the simulations, delivering stunning visual effects.}
    \label{fig:fab}
\end{figure}

==> figures/fig_limitation.tex <==
\begin{figure}[h]
\vspace{-5pt}
    % \raggedleft
    \centering
    \includegraphics[width=0.41\textwidth]{figures/experiments/lim.pdf}
    % \setlength{\abovecaptionskip}{2pt} 
    \caption{\textbf{Limitations of our results.} We present the potential results generated for certain semantics and corresponding viewpoints based on the visual illusion effect.}
    \label{fig:limitation}
\end{figure}
